Extending the RISC-V ISA for Efficient RNN-based 5G Radio Resource Management

Radio Resource Management (RRM) in 5G mobile communication is a challenging problem for which Recurrent Neural Networks (RNN) have shown promising results. Accelerating the compute-intensive RNN inference is therefore of utmost importance. Programmable solutions are desirable for effective 5G-RRM top cope with the rapidly evolving landscape of RNN variations. In this paper, we investigate RNN inference acceleration by tuning both the instruction set and micro-architecture of a micro-controller-class open-source RISC-V core. We couple HW extensions with software optimizations to achieve an overall improvement in throughput and energy efficiency of 15$\times$ and 10$\times$ w.r.t. the baseline core on a wide range of RNNs used in various RRM tasks.

==> RNN/figures/barplot_old.tex <==
\begin{tikzpicture}[scale=0.75]

% \pgfplotsset{
%     calculate offset/.code={
%         \pgfkeys{/pgf/fpu=true,/pgf/fpu/output format=fixed}
%         \pgfmathsetmacro\testmacro{(\pgfplotspointmeta *10^\pgfplots@data@scale@trafo@EXPONENT@y)*\pgfplots@y@veclength)}
%         \pgfkeys{/pgf/fpu=false}
%     },
%     every node near coord/.style={
%         /pgfplots/calculate offset,
%         yshift=-\testmacro
%     },
% }
\begin{axis}[ legend style={draw=none},x tick label style={ /pgf/number format/1000 sep=}, ylabel={Relative Cycle Count vs. RI5CY}, xlabel={RRM Network Model}, enlargelimits=0.1,  ybar, xmin=0, ymajorgrids=true,%ytick={0,100,200,300,400,500}, %xtick={},% ,
xtick=data, legend style={at={(0.5, -0.3), draw=none}, anchor=north,legend columns=-1},
        xticklabels = {
\cite{Challita2017},\cite{Naparstek2017},\cite{ye2018deep},\cite{Sun2017},\cite{Yu2017},\cite{Eisen},\cite{Nasir2018},\cite{Ahmed2018},\cite{Lee2018},\cite{wang2018deep},Avg.
        },
     %   xticklabel style={yshift=-10ex},
     %   major x tick style = {opacity=0},
     %   minor x tick num = 1,
     %   minor tick length=10ex,
       % every node near coord/.append style={
    %            anchor=east,
    %            rotate=90
    %    }
    bar width=0.15, nodes near coords={}, width=0.65\textwidth, height=150,
        ] 

\addplot[cieee0!20!black,fill=cieee0!60!white] table[x index=0,y index=1] {\rnntables{./RNN/tables/}barplot.csv};
\addplot[cieee1!20!black,fill=cieee1!60!white] table[x index=0,y index=2] {\rnntables{./RNN/tables/}barplot.csv};
\addplot[cieee2!20!black,fill=cieee2!60!white] table[x index=0,y index=3] {\rnntables{./RNN/tables/}barplot.csv};
\addplot[cieee3!20!black,fill=cieee3!60!white] table[x index=0,y index=4] {\rnntables{./RNN/tables/}barplot.csv};

% \addplot[cieee0!20!black,fill=cieee0!60!white] table[x index=0,y index=4,restrict expr to domain={\thisrow{show}}{1:1}] {\tables{\rnntables{./RNN/tables/}barplot.csv}};

% \addplot[cieee1!20!black,fill=cieee1!60!white] table[x index=0,y index=5,restrict expr to domain={\thisrow{show}}{1:1}] {\tables{\rnntables{./RNN/tables/}barplot.csv}};

% \addplot[cieee6!20!black,fill=cieee6!60!white] table[x index=0,y index=6,restrict expr to domain={\thisrow{show}}{1:1}] {\tables{\rnntables{./RNN/tables/}barplot.csv}};
  
  %\addplot[color0!20!black,fill=color0!80!white, nodes near coords=Data 1] table [  x=id, y=8x8, col sep=space,restrict expr to domain={\thisrow{show}}{1:1}  ] {tables/area_breakdown.csv};
  
  

%coordinates {(1930,50e6) (1940,33e6) (1950,40e6) (1960,50e6) (1970,70e6)}; 

% \addplot coordinates {(1930,38e6) (1940,42e6) (1950,43e6) (1960,45e6) (1970,65e6)}; 

%\addplot coordinates {(1930,15e6) (1940,12e6) (1950,13e6) (1960,25e6) (1970,35e6)}; 

%\addplot[red,sharp plot,update limits=false] coordinates {(1910,4.3e7) (1990,4.3e7)}; 


\legend{RI5CY, {+(Out)-FM-Tiling}, {+VLIW+tanh+sig Extensions}, +In-FM-Tiling} 
\end{axis} \end{tikzpicture}
